SCINeRF: Neural Radiance Fields from a Snapshot Compressive Image

In this paper, we explore the potential of Snapshot Compressive Imaging (SCI) technique for recovering the underlying 3D scene representation from a single temporal compressed image. SCI is a cost-effective method that enables the recording of high-dimensional data, such as hyperspectral or temporal information, into a single image using low-cost 2D imaging sensors. To achieve this, a series of specially designed 2D masks are usually employed, which not only reduces storage requirements but also offers potential privacy protection. Inspired by this, to take one step further, our approach builds upon the powerful 3D scene representation capabilities of neural radiance fields (NeRF). Specifically, we formulate the physical imaging process of SCI as part of the training of NeRF, allowing us to exploit its impressive performance in capturing complex scene structures. To assess the effectiveness of our method, we conduct extensive evaluations using both synthetic data and real data captured by our SCI system. Extensive experimental results demonstrate that our proposed approach surpasses the state-of-the-art methods in terms of image reconstruction and novel view image synthesis. Moreover, our method also exhibits the ability to restore high frame-rate multi-view consistent images by leveraging SCI and the rendering capabilities of NeRF. The code is available at https://github.com/WU-CVGL/SCINeRF.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/n_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.


==> sec/result_sup2.tex <==
\begin{figure*}[htb]


\vspace{-0.25cm}
\begin{minipage}[c]{1.0\textwidth}
\begin{minipage}[c]{\linewidth}
\centering
  \begin{minipage}[c]{0.14\linewidth}
  \centering
  \small
  \ \\  Measurement~
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \centering
  \small
  \ \\ NeRF\cite{mildenhall2021nerf}+\\GAP-TV~\cite{yuan2015generalized}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \centering
  \small
  \ \\ \ NeRF\cite{mildenhall2021nerf}+\\PnP-FFDNet~\cite{yuan2020plug}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \centering
  \small
  \ \\ \ NeRF\cite{mildenhall2021nerf}+\\EfficientSCI~\cite{wang2023efficientsci}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \centering
  \small
  \ \\ \ Ours
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \centering
  \small
  \ \\ \ Ground Truth
  \end{minipage}
\end{minipage}
\\
\begin{minipage}[c]{\linewidth}
\centering
  \begin{minipage}[c]{0.14\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig2_input.jpg}
  
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig2_tv.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig2_ffd.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig2_esci.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig2_ours.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.14\linewidth}
  \includegraphics[width=1\linewidth]{figures/fig2_gt.jpg}
  \end{minipage}
\end{minipage}
\end{minipage}
\\
    \vspace{-0.25em}
   \caption{\textbf{Qualitative evaluations of our method against NeRF+SOTA methods.} We compared the quality of synthesized novel-view images from our SCINeRF against that of vanilla NeRF with reconstructed images from state-of-the-art methods. Top to bottom shows different scenes including \textit{Airplants, Hotdog, Cozy2room}, \textit{Tanabata}, \textit{Factory} and \textit{Vender}. The qualitative comparisons demonstrate that our SCINeRF outperforms existing approaches.  
   }
   \label{sfig2}
    %\vspace{-0.8em}
   
\end{figure*}

==> sec/result_sup3.tex <==
\begin{figure*}[!tb]


%\hspace{-0.25cm}
\begin{minipage}[c]{1.0\textwidth}
\begin{minipage}[c]{\linewidth}
\centering
  \begin{minipage}[c]{0.155\linewidth}
  \centering
  \small
  \ \\  Measurement~
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \centering
  \small
  \ \\ GAP-TV~\cite{yuan2015generalized}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \centering
  \small
  \ \\ \ PnP-FFDNet~\cite{yuan2020plug}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \centering
  \small
  \ \\ \ EfficientSCI~\cite{wang2023efficientsci}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \centering
  \small
  \ \\ \ Ours
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \centering
  \small
  \ \\ \ Original Scene
  \end{minipage}
\end{minipage}
\\
\begin{minipage}[c]{\linewidth}
\centering
  \begin{minipage}[c]{0.155\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig3_input9.jpg}
  
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig3_tv9.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig3_ffd9.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig3_esci9.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig3_ours9.jpg}
  \end{minipage}
  ~
  \begin{minipage}[c]{0.155\linewidth}
  \includegraphics[width=1\linewidth]{figures/sfig3_gt9.jpg}
  \end{minipage}
\end{minipage}
\end{minipage}
\\

   \caption{\textbf{Qualitative evaluations of our method against SOTA SCI image restoration methods with real dataset.} Top to bottom shows different scenes. Since compressed ground truth images are unavailable, we captured separate scene images after capturing SCI measurement. The qualitative comparisons demonstrate that our SCINeRF surpasses prior methods on image reconstruction with real dataset.  
   }
   \label{sfig3}
    %\vspace{-0.8em}
   
\end{figure*}
